NDNTP: A Named Data Networking Time Protocol

Named Data Networking (NDN) architectural features, including multicast data delivery, stateful forwarding, and in-network data caching, have shown promise for applications such as video streaming and file sharing. However, collaborative applications, requiring a multi-producer participation introduce new NDN design challenges. In this paper, we highlight these challenges in the context of the Network Time Protocol (NTP) and one of its most widely-used deployments for NTP server discovery, the NTP pool project. We discuss the design requirements for the support of NTP and NTP pool and present general directions for the design of a time synchronization protocol over NDN, coined Named Data Networking Time Protocol (NDNTP).

==> distance_probing.tex <==
\section{Distance-Based Server Selection}
\label{sec:prob}
%\TODO{Again this section is wrong!!! NTP does not do anything about geolocations!! NTP Pool does!!!!! We did not do experiments with just NTP. The experiments were with NTP pool!!!}

While NDN inherently supports reaching the closest server that offers a given service (\eg time synchronization), there might be cases, where occasionally reaching distant servers within a zone may be desirable for a time synchronization protocol in order to: (i) reduce targeted attacks, where entities controlling a group of neighboring servers return bogus timestamps; and (ii) enable load balancing among nearby and distant servers. Reaching servers within similar distances from a client may also be desirable in order to reduce jitter in round-trip delays. %by having requests reach servers within similar distances.

%NTP pool makes use of IP geolocations for the discovery of servers geographically close to clients and relies on DNS for load-balancing among servers. 
To investigate whether NTP pool shares the above objectives as well as better understand how it operates, we performed a set of preliminary experiments. Specifically, we deployed NTP clients--two in North America (in Missouri and New Mexico) and one in Europe (in Athens, Greece)--and we configured them to have their time synchronized through NTP pool. Each client queries four NTP pool servers (\ie the default number of servers for NTP) every minute over a 24-hour period.

%NTP requests from different clients during a 24-hour period and show the NTP servers probed and their characteristics. We use three Linux machines; two in North America (New Mexico and Missouri) and another client in Europe (Greece) to run a script that queries four (\ie the default) different servers: {\tt ntp command we've used}. 

% \begin{figure}[t]
% \centering
%  \begin{subfigure}[b]{0.9\linewidth}
%  \includegraphics[width=\textwidth]{figures/IP_CDF_log.eps}
%  \caption{CDF log}
%  \label{IP_cdf_log}
%  \end{subfigure} \\
%  \begin{subfigure}[b]{0.9\linewidth}
%  \includegraphics[width=\textwidth]{figures/IP_CDF.eps}
%   \caption{CDF}
%   \label{IP_cdf}
%  \end{subfigure}%\hfil
%  \caption{I will change the format of this figure!!}% 100, 250, 500, and 1000}
%  \label{IP_cdf_all}
% \end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/IP_CDF_combo-eps-converted-to.pdf}
    \caption{Distribution of server occurrences; servers are sorted from the most probed to the least probed in the New Mexico (NM), Missouri (MO) and Athens (Ath) traces. The inside plot is in log scale zooming in the distribution of the most popular servers}
    \label{IP_cdf_all}
\end{figure}


Figure~\ref{IP_cdf_all} illustrates the CDF of the unique NTP pool servers (sorted by popularity--number of times a server is probed in the trace) in the three traces.
We notice that both north American traces have very similar trends characterized by almost identical CDF distributions, while the European trace has very different properties. Based on the European trace, the unique servers probed are $20 \times$ fewer than those probed in North American--14 unique servers in the trace from Athens compared to 229 and 300 in the New Mexico and the Missouri traces respectively. Our understanding is that this is due to the difference in the NTP pool zone sizes for North America and Europe--at the time of the experiments, there were $3.1 \times$ more NTP pool servers in Europe than in North America.

Moreover, we found that the servers probed from Athens are closer to the client than those probed from New Mexico and Missouri. Specifically, more than 80\% of the servers probed from Athens are within 50 kilometers from the client, while less than 10\% of the servers probed from New Mexico are 1000 kilometers from the client (\ie $250 \times$ further than the 50 kilometers neighboring circle in Athens).

\begin{figure*}[t]
\centering
 \begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\textwidth]{figures/ath_CDF-eps-converted-to.pdf}
 \caption{Athens}
 \label{dist_ath}
 \end{subfigure}
 \begin{subfigure}[b]{0.32\linewidth}
 \includegraphics[width=\textwidth]{figures/nmsu_CDF-eps-converted-to.pdf}
  \caption{New Mexico}
  \label{dist_nmsu}
 \end{subfigure}%\hfil
  \begin{subfigure}[b]{0.32\linewidth}
  \includegraphics[width=\textwidth]{figures/umsl_CDF-pdf-crop.pdf}
  \caption{Missouri}
  \label{dist_umsl}
 \end{subfigure}%\hfil
 \caption{CDF of average distances (AVG) and standard deviations (STD) per run in (a) Athens, (b) New Mexico, and (c) Missouri datasets}% 100, 250, 500, and 1000}
 \label{distance_cdf}
\end{figure*}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/ath_CDF.eps}
%     \caption{Athens distances to servers}
%     \label{fig:ath_distance}
% \end{figure}

We illustrate in Figure~\ref{distance_cdf} the average distances (in kilometers) and the standard deviation per run of the NTP protocol (\ie four servers are probed per run) from (a) Athens, (b) New Mexico, and (c) Missouri respectively. First, we notice that the four servers probed in each run tend to have similar distances from the client as shown by the lower values in standard deviation distributions of Figure~\ref{distance_cdf}. Furthermore, we show that in almost 40\% of the runs of the Athens trace, requests reached all four servers within the same distance of 45 to 50 kilometers. On the other hand, the four servers probed in each run of the New Mexico trace have different distances from the client, resulting in larger standard deviations. Our understanding is that this is due to the larger physical surface of the North America zone, compared to Europe, in general, and Greece as a country, in particular.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/nmsu_IP_CDF.eps}
%     \caption{NMSU IPs}
%     \label{fig:nmsu_ip}
% \end{figure}

\subsection{Lessons Learned} 

The lessons learned from these preliminary experiments fall into three main categories: (i) {\em zone probing}: NTP pool employs a zone probing scheme that consists of reaching (nearby and occasionally more distant) NTP servers from within the client's zone; (ii) {\em similar distance probing}: most servers probed in each run of the NTP protocol are within similar distances from the client, thus responses return to the client with similar delays; and (iii) {\em reaching a different set of NTP servers in each run}: NTP clients that make use of NTP pool reach, in general, a different set of servers every time. Our data showed that in North America servers are rarely selected more than few times in the 24-hour period. In smaller zones, such as in Athens, where the number of NTP servers in the zone is small, servers are probed multiple times. Servers from distant zones are also probed, although infrequently (Figure~\ref{distance_cdf}), to reduce the reliance on a small subset of servers that may form a collaborative malicious group (collusion attacks).

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/nmsu_CDF.eps}
%     \caption{NMSU distances to servers}
%     \label{fig:nmsu_cdf}
% \end{figure}

\subsection{Design Directions}

%\TODO{People can criticize that NTP pool does geo distance, but we do hops and these 2 things are not the same}

From the lessons learned from our preliminary experiments and the NTP pool description (Figure~\ref{fig:ntp}), \sol needs to be able to reach servers within a given ``{\em zone}'' and within controlled distances for the requests of the same protocol run. While a zone in an IP-based NTP pool design refers to a country or a region, which can be limited in size and may introduce delays in larger zones, we define a zone as the region within a certain number of hops from a client. For instance, a client in New Mexico will be able to reach servers within $h$ hops making the case of reaching servers in New Mexico as likely as reaching servers in other states of North America.

%Expanding NDN to support reaching ``further'' servers is required.


This can be achieved through the deployment of stateful forwarding modules that enable reaching not only closest servers from clients but also ``further'' servers. We propose two client-based solutions that enables client to get fine-grained control over how far his/her message travels.

One design direction consists of using the \emph{hop limit} field of Interest packets. Clients requiring requests to reach servers at least $h hops$ away, add the value $h$ to this field. Each hop forwarder decrements the hop limit value of \sol Interests and forward the Interest using the outgoing interface that has the highest cost--in NDN outgoing interfaces for a given name prefix have a cost and the lower the cost the closest the server (or the shorter the RTT). When this value reaches 1, the forwarding strategy resets the value to {\tt NULL} and switches to the {\tt best route} forwarding strategy that tries to reach the closest servers. Using this solution all probed servers are at least h hops away from the client, thus delays would be similar.

Another design direction consists of enabling clients to include a probability to the Interest name. The lower the probability, the higher the cost of the interface chosen by the forwarding strategy. For instance, \name{/NTP/time/P=0.3} sent by clients would be interpreted by forwarders such that they choose the worst cost with a probability of 0.7 and the best interface towards the server with probability 0.3. While this method is simple and does not require any change of the structure of the Interests in NDN, it does not ensure reaching servers at a given distance (or at least h hops from) from the requester, however it will allow client's fine-grained control of when request must reach closer servers vs. randomly probing servers away.






%  These modules will be aware of how far (in terms of hops) \sol servers are, ensuring that servers within $h$ hops from the client are reached. To achieve that, forwarders utilize the \emph{hop limit} field of Interest packets, assuming that they are aware of how far (in terms of hops) \sol servers are from them (we discuss alternative solutions to achieve that below). Specifically, clients select the hop limit value of their \sol Interests, while each hop forwarder decrements the hop limit value of these Interests--when this value reaches zero, the Interest is discarded by the network. As a result, forwarders will be able to forward \sol requests for the same run across similar distances at most $h$ hops away from clients.

% To make forwarders aware of how far (distance in terms of hops) \sol servers are from them, the distance information can be propagated via a routing protocol. Another solution would be to augment \sol responses so that they carry a field, which indicates the number of hops from the server. The value of this field will be incremented by each forwarder on the return path of the response back to the client. In this way, forwarders will be able to know their distances from the available servers. 

%by utilizing the \emph{hop limit} field of Interests. Clients specify the hop limit value of their \sol Interests, while each hop forwarder decrements the hop limit value of these Interests.

%This solution requires adding a {\tt NumberOfHop} field to the interest packet in NDN. The forwarding strategy will decrease the number in this field, and the router that receives an Interest with {\tt NumberOfHop=0} tries to reach the closes server. Using this solution all probed servers will be at similar distances (measured in the number of hops) from the consumer, thus delays would be similar.

% \TODO{I cannot make sense out of this paragraph. I suggest we comment out.}
% Alternatively, clients include a probability to the Interest name. The lower the probability, the higher the cost of the face chosen by the forwarding strategy. For instance, \name{/NTP/time/P=0.3} sent by clients would be interpreted by forwarders such that they choose the worst cost with a probability of 0.7 and the best face towards the server with probability 0.3. While this method does not change the structure of the Interests in NDN, it does not ensure ``same'' distance from the requester, however it will ensure random probing of servers within a given zone.  



% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{figures/distance-CDF.eps}
%     \caption{CDF distance}
%     \label{fig:cdf_distance}
% \end{figure}



% \begin{figure}[t]
% \centering
%  \begin{subfigure}[b]{0.9\linewidth}
%  \includegraphics[width=\textwidth]{figures/IP_CDF_log.eps}
%  \caption{CDF log}
%  \label{IP_cdf_log}
%  \end{subfigure} \\
%  \begin{subfigure}[b]{0.9\linewidth}
%  \includegraphics[width=\textwidth]{figures/IP_CDF.eps}
%   \caption{CDF}
%   \label{IP_cdf}
%  \end{subfigure}%\hfil
%  \caption{}% 100, 250, 500, and 1000}
%  \label{IP_cdf}
% \end{figure}

==> future-directions.tex <==
\section {Network Time Synchronization: Future Directions}

\subsection {In-Network Computing for Time Synchronization}

\subsection {Information-Centric Time Synchronization}

==> multi-producer-backup.tex <==
\section{Enabling Multi-Server Time Sample Fetching}
\label{sec:multi-server}

The best current practices of NTP deployment~\cite{reilly2017network} indicate that a client should: (i) contact more than one NTP servers; and (ii) collect multiple time samples from each NTP server. The NDN communication model is inherently multipath/multicast supporting requirement (i), since an Interest can be forwarded towards multiple producers (\ie NTP servers in our case). However, deterministically contacting the same server multiple times in the context of requirement (ii) is counter-intuitive to the purpose of NDN, where data can be retrieved from any party that can provide it. That is, the NDN architecture itself does not provide any explicit mechanisms to guarantee that Interests will be forwarded along a specific path towards a certain server. %Moreover, NDN forwarders accept only a single data packet for each Interest--the first returning data packet will consume the corresponding PIT entry, while any subsequent data packet will be dropped.  

\emph{Design directions:} We present a wide spectrum of design directions ranging from solutions of unicast nature to multicast ones.

%We categorize our proposed directions to design a multi-server fetching scheme into two: (i) ..... and (ii) .....

\subsection{Directions for solutions of unicast nature}
\label{sec:unicast}
 
A solution would be the use of techniques to create labels of paths that Interests should take~\cite{moiseenko2017path}. Each Interest will carry such a label--at each hop, NDN forwarders will forward an Interest based on this label, which determines the next-hop(s) that an Interest should take. At the beginning of their operation, NTP clients will perform a path discovery process, where they will acquire a label for a path to a server. This process will end when a client acquires a label for the desired number of different servers. As a result, the client uses the same path label to collect different samples from the same server, since Interests carrying the same label will be forwarded across the same path. Note that the process of discovering multiple paths still requires forwarders to receive multiple data packets (one per discovered path), aggregate them into a single packet, and forward the aggregated packet back to the their previous hop.

Another solution would be to utilize the stateful NDN forwarding plane, without the need for forwarders to aggregate multiple NTP responses from servers and send aggregated responses back to clients. Forwarding modules can be created and deployed on NDN forwarders, so that Interests for time samples from the same NTP server can be forwarded towards this server. Specifically, NTP clients create a ``session-like'' paradigm with a specific server, so that they can request multiple time samples from it. An example namespace to achieve that is illustrated in Figure~\ref{figure:namespace}. The name prefix includes the NTP name prefix (\name{/NTP/time}), followed by: (i) \emph{a random hash} to by-pass the aggregation of requests from different clients as further discussed in Section~\ref{sec:others} (each different hash identifies a set of sessions initiated by a client); (ii) \emph{a session number} that identifies a specific session with an NTP server; and (iii) \emph{a sample number} that identifies a specific time sample requested from an NTP server.

When an NDN forwarder receives an NTP request, it dispatches it to the corresponding forwarding module. This module identifies requests from the same client but from different sessions. In this way, time sample requests for the same session number are forwarded along the same path, so that they reach the same NTP server. 

\begin{figure}[h]
\centering
\includegraphics[width=0.9\linewidth]{figures/namespace.pdf}
\caption{Namespace for the collection of multiple time samples from the same \sol server}
\label{figure:namespace}
\end{figure}

\subsection{Directions for solutions of multicast nature}

The solutions mentioned in Section~\ref{sec:unicast} can be extended to support multicast Interest forwarding. 

During the discovery process of paths performed by clients, the path labels can be constructed to include multiple next hops at each router. As a result, client Interests will be forwarded along multiple different paths, potentially reaching multiple different servers. 

\TODO{Abde, add your text about how we extend the stateful forwarding plane for Interest multicasting here}

A challenge arises for both approaches when data packets are returned back to clients. NDN forwarders accept only a single data packet for each Interest--the first returning data packet will consume the corresponding PIT entry, while any subsequent data packet will be dropped. 

To tackle this challenge, one direction would be to enhance the NDN communication model, so that forwarders can accept multiple data packets (one per interface that a corresponding Interest was forwarded through). These data packets will be aggregated into a single packet, which will be forwarded back to the forwarder's previous hop. In this way, forwarders can multicast NTP requests towards multiple servers, receive response from multiple servers and aggregate them into a single response, which will eventually be received by the NTP client. Note that this enhancement does not invalidate NDN's architectural principle of ``flow balance'', that is, one Interest will still bring one data packet back at each hop forwarder. However, it can take arbitrarily long for a forwarder to collect multiple data packets through different paths, since the length of each path might be different. This could impede the precision of the time synchronization process, since it skews the round-trip delay measurements of clients.

An alternative direction would be consume each \sol related PIT entry only after all the responses have been received. Specifically, a PIT entry at a forwarder will stay alive and bring back one data packet for each outgoing interface the corresponding \sol Interest was forwarded through. This would help clients to collect accurate round-trip delay measurements and improve the precision of the time synchronization process. However, it would break the NDN ``flow balance'' principle.

==> ntp-ndn-design-new.tex <==
\section {NTP over NDN: Opportunities and Challenges}
\label{sec:design}

In this section, we first give an overview of the network model. We then present a set of NDN features that need rethinking for the design of an NTP-like protocol over NDN including a set of challenges and design directions to overcome these challenges. %We also discuss additional directions/considerations for the design of an NTP-like protocol in NDN.

\subsection {Network Model}

%Here we need to say we have a network with a number of NTP servers that announce a prefix \name{/NTP/time} and then a bunch of clients that want to do time sync. Talk about the overall design space in general.

We assume that there is a number of NTP servers acting as NDN data producers. The servers receive NTP requests (Interest packets) under the \name{/NTP/time} namespace sent by NTP clients acting as data consumers. Servers respond to requests by generating and signing NTP responses (data packets), which contain the current timestamp and other necessary fields as determined by the NTP protocol specification~\cite{mills2010network}. NTP clients are inter-connected with servers through one or more hops (\ie one or more NDN forwarders). NTP servers announce the \name{/NTP/time} namespace to the network--a named-based routing protocol (\eg NLSR~\cite{hoque2013nlsr}) is used to propagate this server namespace announcement and establish routes towards the server (\ie install the proper forwarding information on NDN forwarders). 

\subsection {Control over Interest aggregation and in-network caching}

Interest aggregation and in-network caching are two fundamental properties of the NDN architecture. However, they pose challenges to the design of an NTP-like protocol over NDN. We discuss specific related challenges and propose directions to resolve them below.

%\begin {itemize}[leftmargin=0cm,itemindent=.3cm,align=left]

\noindent \textbf {Challenge 1:} How to avoid stale cached NTP timestamps? 

In NDN, data caching is a feature natively supported by the network architecture. However, the NTP clients are in need of accurate time precision. In-network caching poses a challenge to acquiring accurate up-to-date timestamps, since there is no way for a client to know whether an NTP response was received from an NTP server or a CS. Moreover, an NTP response retrieved from a CS makes it hard for NTP clients to predict when this response was generated, since the client does not know for how long the response has been cached.

\emph{Design directions:} To avoid fetching cached NTP responses, NTP servers set the value of the Freshness Period field of the responses they generate to a reasonably low value (or even 0), indicating that NTP responses will become (almost) instantly stale once they are cached in the network. Subsequently, NTP clients send NTP Interests that contain the MustBeFresh field in order to avoid retrieving stale cached NTP responses~\cite{mastorakis2018real}.

\noindent \textbf {Challenge 2:} How to ``by-pass'' Interest aggregation in PIT to avoid clock skew?

The PIT aggregation of Interests with the same name can pose another challenge for clients to receive accurate timestamps. Given that NTP relies on clients measuring the round-trip delays to servers, Interest aggregation can skew the round-trip delay measurements of clients, and, subsequently, their clock. 

\emph{Design directions:} To address this challenge, NTP clients randomize the name of their Interests, so that they avoid aggregation in PIT. This can be achieved by attaching a random hash in the Interest name. However, there is yet another challenge on where in the name this random hash should be. Given that the name prefix of Interests is used for forwarding purposes, the randomization should happen in the Interest name suffix. We present specific examples of the NTP namespace design in the next challenge.

\subsection {One Interest brings one data packet back for all outgoing interfaces}

\TODO {The title of this subsection is misleading for the time being.. I do not personally see how to turn this subsection into what the title indicates.. Abde, this is your idea.. Please help..}

In NDN, Interests can be forwarded towards one or more next-hops (through one or more interfaces) by NDN forwaders. However, only one data packet for all outgoing interfaces can be returned for each Interest by a forwarder. This poses challenges for communication use-cases such as NTP, where the best current practices indicate that a client should: (i) contact more than one NTP servers; and (ii) collect multiple time samples from each NTP server.

\noindent \textbf {Challenge:} How to send NTP requests to multiple different servers and how collect multiple time samples from each one of them?

The inherently multi-path communication model of NDN can facilitate contacting multiple NTP servers. However, deterministically contacting the same server multiple times is counter-intuitive to the purpose of NDN, where data can be retrieved from any party that can provide it. That is, the NDN architecture itself does not provide any explicit mechanisms to guarantee that Interests will be forwarded along a specific path towards a certain server.

\emph{Design directions:} One direction would be to enhance the NDN communication model, so that forwarders can receive multiple data packets (one per interface that a corresponding Interest was forwarded through), aggregate them into a single packet, and forward this aggregated packet back to the their previous hop. In this way, forwarders can multicast NTP requests towards multiple servers, receive response from multiple servers and aggregate them into a single response, which will eventually be received by the NTP client. Note that this enhancement does not invalidate NDN's architectural principal of ``flow balance'', that is, one Interest will still bring one data packet back at each hop forwarder.
 
Techniques can be used to create labels of paths that Interests should take~\cite{moiseenko2017path}. Each Interest will carry such a label--at each hop, NDN forwarders will forward an Interest based on this label, which determines the next-hop(s) that an Interest should take. At the beginning of their operation, NTP clients will perform a path discovery process, where they will acquire a label for a path to a server. This process will end when a client acquires a label for the desired number of different servers. As a result, the client uses the same path label to collect different samples from the same server, since Interests carrying the same label will be forwarded across the same path. Note that the process of discovering multiple paths still requires forwarders to receive multiple data packets (one per discovered path), aggregate them into a single packet, and forward the aggregated packet back to the their previous hop.

Another direction would be to utilize the stateful NDN forwarding plane, without the need for forwarders to aggregate multiple NTP responses from servers and send aggregated responses back to clients. Forwarding modules can be created and deployed on NDN forwarders, so that Interests for time samples from the same NTP server can be forwarded towards this server. Specifically, NTP clients create a ``session-like'' paradigm with a server to request multiple time samples from it. An example namespace to achieve that is illustrated in Figure~\ref{figure:namespace}. The name prefix includes the NTP name prefix (\name{/NTP/time}), followed by: (i) \emph{a random hash} to by-pass the aggregation of requests from different clients (each different hash identifies a set of sessions initiated by a client); (ii) \emph{a session number} that identifies a specific session with an NTP server; and (iii) \emph{a sample number} that identifies a specific time sample requested from an NTP server.

When an NDN forwarder receives an NTP request, it dispatches it to the corresponding forwarding module. This module identifies requests from the same client but from different sessions. In this way, time sample requests for the same session number are forwarded along the same path, so that they reach the same NTP server. 

\TODO{Add more stuff on how this strategy works once we figure out the details..}

\begin{figure}[h]
\centering
\includegraphics[width=0.9\linewidth]{figures/namespace-crop.pdf}
\caption{Namespace for the collection of multiple time samples from the same NTP server}
\label{figure:namespace}
\end{figure}

%\end{itemize}




==> related.tex <==
\section{Related Work}

%\TODO{What kind of related work should we add here? People have done related work on NTP in general and in security specifically. Have not seen any related work on time sync over NDN/ICN. One point we could make is that CCN assumes a synchronized clock among the communicating parties.}

The community has worked on adapting a number of IP-based services/applications to run on top of NDN, while general guidelines on adapting non-NDN applications to operate on an NDN network have also been investigated~\cite{liang2018ndnizing}. For example, peer-to-peer file sharing applications such as BitTorrent~\cite{mastorakis2017ntorrent} and online multi-player games such as Minecraft~\cite{moll2019distributing} have been adapted to operate on top of an NDN network substrate. Moreover, infrastructure services, such as DNS~\cite{afanasyev2017ndns} have been re-designed to operate on top of an NDN network. However, a service to provide time synchronization in NDN to applications, systems, and devices that may need it remains a largely unexplored area.

==> security.tex <==
\section{\sol Security}

\sol utilizes NDN's network-layer security principles for response authentication purposes. Specifically, clients based on the signature of responses can: (i) verify that responses have not been spoofed (\eg due to man-in-the-middle attacks); and (ii) decide whether they trust the servers that generated responses based on a pre-established set of trust anchors~\cite{zhang2018overview}. However, this does not protect against servers that become malicious over time (\eg due to a security breach). 

\emph {Design directions:} As discussed in Section~\ref{sec:multi-server}, clients may receive time samples from multiple different servers, thus they are able to identify servers that provide inaccurate timestamps. In this way, clients use labels of paths that take their requests to servers providing accurate timestamps or let the network know, so that future requests are forwarded towards different directions (\ie towards different servers).

%One direction would be for clients to create communication groups for time synchronization with a number of servers. This requires the participants in a group to announce a group name prefix, which will be used for communication purposes.

\TODO{What else to write here?}
